Angles from B Decays with Charm: Summary of Working Group 5 of the CKM Workshop 2006

We summarize the results presented in Working Group 5 (WG5) of the CKM 2006 Workshop in Nagoya. The charge of WG5 was to discuss the measurements of unitarity triangle angles $\beta/\phi_1$ and $\gamma/\phi_3$ from $B$-meson decays containing charm quark(s) in the final states.

==> abstract.tex <==
We summarize the results presented in Working Group 5 (WG5) of the CKM 
 2006 Workshop in Nagoya. The charge of WG5 was to discuss the measurements 
 of unitarity triangle angles $\beta/\phi_1$ and $\gamma/\phi_3$ from $B$-meson 
 decays containing charm quark(s) in the final states. 


